P2P-Bridge: Diffusion Bridges for 3D Point Cloud Denoising

In this work, we tackle the task of point cloud denoising through a novel framework that adapts Diffusion Schr\"odinger bridges to points clouds. Unlike previous approaches that predict point-wise displacements from point features or learned noise distributions, our method learns an optimal transport plan between paired point clouds. Experiments on object datasets like PU-Net and real-world datasets such as ScanNet++ and ARKitScenes show that P2P-Bridge achieves significant improvements over existing methods. While our approach demonstrates strong results using only point coordinates, we also show that incorporating additional features, such as color information or point-wise DINOv2 features, further enhances the performance. Code and pretrained models are available at https://p2p-bridge.github.io.

==> figures/arkit_qualitative.tex <==



\begin{figure}[ht!]
\begin{center}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{rcl}
Noisy &\includegraphics[width=0.6\linewidth, height=8px]{figures/color_gradient.png} & Clean
    \end{tabular}
}
\end{center}

\newcommand{\tabspacesnpp}{0.16}

\begin{center}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/421383_42444966/iphone/iphone_iphone.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/421383_42444966/bilateral/bilateral_iphone_R=0.1_r=0.1_N=1_n=0.04.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/421383_42444966/SD/SD_denoised.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/421383_42444966/PDF/PDF_denoised.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/421383_42444966/P2SB/P2SB_PVDL-ARK-XYZ_iphone_100000_5_ema.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/421383_42444966/gt/gt_faro.jpg}
\\
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/466183_45260920/iphone/iphone_iphone.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/466183_45260920/bilateral/bilateral_iphone_R=0.1_r=0.1_N=1_n=0.04.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/466183_45260920/SD/SD_denoised.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/466183_45260920/PDF/PDF_denoised.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/466183_45260920/P2SB/P2SB_PVDL-ARK-XYZ_iphone_100000_5_ema.jpg}
\includegraphics[width=\tabspacesnpp\linewidth,clip]{figures/arkit_eval/466183_45260920/gt/gt_faro.jpg}
\\


\end{center}
\setlength{\tabcolsep}{2pt}
\vspace{-15px}
\resizebox{\textwidth}{!}{
\hspace{0px}\begin{tabular}{cccccc}
\hspace{0.25\linewidth} &
\hspace{0.25\linewidth} &
\hspace{0.25\linewidth} &
\hspace{0.25\linewidth} &
\hspace{0.25\linewidth} &
\hspace{0.25\linewidth} \\
     \textbf{Noisy Input} & \textbf{Bilateral}\cite{digne_bilateral} &\textbf{ScoreDenoise}\cite{score_denoise} & \textbf{PD-Flow}\cite{mao2022pd} & \textbf{\name{}} & \textbf{Ground-Truth} \\
     &&&& \textbf{(Ours)} &\textbf{(Faro)} \\ 
\end{tabular}
}
\caption{Qualitative comparison on ARKitScenes \cite{dehghan2021arkitscenes} using the ARKit iPhone reconstructions as noisy input to the denoising methods.}
\label{fig:argit_qualitative}
\end{figure}

==> tables/arkit.tex <==
\begin{wraptable}{r}{0.4\textwidth}
    \centering
	\caption{
		\textbf{ARKitScenes Scores.}
		Quantitative point cloud denoising comparisons on a subset of the ARKitScenes \cite{dehghan2021arkitscenes} test set. The Faro scanner point clouds act as a reference for the ground truth. All metrics are multiplied by $10^3$.}
    \resizebox{\columnwidth}{!}{%
	\begin{tabular}{lccccccc}
		\toprule
		Method                            & Features       & $\cdforw$ & $\cdbakw$ & CD        \\
		\midrule
		Bilateral \cite{digne_bilateral}  & XYZ            & 15.87     & 70.49     & 43.18     \\
		DMR \cite{luo2020differentiable}  & XYZ            & 10.84     & \rd 30.51 & 20.68     \\
		ScoreDenoise \cite{score_denoise} & XYZ            & \rd 9.56  & 30.86     & 20.21     \\
		MAG \cite{zhao2023point}          & XYZ            & \st 9.57  & 30.82     & 20.20     \\
		PD-Flow \cite{mao2022pd}          & XYZ            & 9.93      & 33.82     & 21.87     \\
		\textbf{\name{} Ours}                      & XYZ            & \nd 9.65  & 30.64     & \rd 20.14 \\
		\midrule
		\textbf{\name{} Ours}                      & XYZ, RGB       & \nd 9.65  & \nd 30.45 & \nd 20.05 \\
		\textbf{\name {} Ours}                     & XYZ, RGB, DINO & \st 9.57  & \st 30.27 & \st 19.92 \\
		\bottomrule
	\end{tabular}%
    }
	\label{tab:evaluation_arkit}
\end{wraptable}


==> tables/backbone_analysis.tex <==
\begin{table}[ht]
    \centering
    \caption{Evaluation of different diffusion model backbones trained for 50k steps on a small subset of ScanNet++. CD and P2M are both multiplied by $10^4$.}
    \begin{tabular}{lcc}
        \toprule
         Backbone & CD & P2M\\
         \midrule
         Minkowksi \cite{minkowksi_4d} & \rd 12.79 & \rd 32.39\\
         SetTransformer \cite{tyszkiewicz2023gecco} & \nd 10.50 & \nd 15.46\\
         PVCNN \cite{pvcnn} & \st 9.76 & \st 14.33\\
         \bottomrule
    \end{tabular}%
    \label{tab:backbone_analysis} 
\end{table}



==> tables/bridge_ablation.tex <==
\begin{minipage}[ht!]{.29\linewidth}
      \captionof{table}{Bridge settings comparison on the PU-Net dataset. CD and P2M are multiplied by $10^4$.}
    \resizebox{\columnwidth}{!}{%
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{cccc}
        \toprule
         OT-ODE & Alignment &  CD & P2M\\
         \midrule
         \cmark &  \xmark & 49.33 & 44.22\\
         \cmark &  \cmark & 2.11  & 0.65\\
         \xmark & \cmark & 2.45 & 0.73\\
         \bottomrule
    \end{tabular}}
   \label{tab:bridge_ablation}
\end{minipage}

==> tables/network_ablation.tex <==
\begin{table}[ht]
    \centering
    \captionof{table}{Network configuration study on ScanNet++. SE describes squeeze-and-excitation blocks after convolutional layers, introduced in \cite{hu2018squeeze}. CD and P2M are multiplied by $10^4$.}
    \vspace{-8px}
    \resizebox{.75\columnwidth}{!}{%
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{ccccccc}
        \toprule
         Base Channels & PVC Blocks & Global Feature & SE & Feature Embedding & CD ($\Delta$)& P2M ($\Delta$)\\
         \midrule
         32 & 1222 & \cmark & \cmark & \cmark & 9.41 $(+1.14)$& 13.78 $(+4.08)$\\
         32 & 2122 & \cmark & \cmark & \cmark & 9.45 $(+1.18)$& 13.82 $(+4.12)$\\
         32 & 2212 & \cmark & \cmark & \cmark & 9.33 $(+1.06)$& 13.70 $(+4.00)$\\
         32 & 2221 & \cmark & \cmark & \cmark & 9.32 $(+1.05)$& 13.70 $(+4.00)$\\
         32 & 2222 & \cmark & \cmark & \cmark & 9.26 $(+0.99)$& 13.67 $(+3.97$\\
         \midrule
         32 & 2222 & \xmark & \cmark & \cmark & 9.36 $(+1.09)$& 13.75 $(+4.05)$\\
         32 & 2222 & \cmark & \xmark & \cmark & 9.33 $(+1.06)$& 13.71 $(+4.01)$\\
         32 & 2222 & \cmark & \cmark & \xmark & 9.76 $(+1.49)$& 14.33 $(+4.61)$\\
         \midrule 
         64 & 2222 & \cmark & \cmark & \cmark & 8.31 $(+0.04)$& 9.72 $(+0.02)$\\
         64 & 2322 & \cmark & \cmark & \cmark & $\mathbf{8.27~(--)}$ & $\mathbf{9.70~(--)}$\\
         \bottomrule
    \end{tabular}%
    }
    \label{tab:network_ablation}
\end{table}





==> tables/scannetpp.tex <==
\begin{table}[htb!]
	\caption{
		\textbf{ScanNet++ Scores.}
		Quantitative point cloud denoising comparisons on a subset of the ScanNet++ \cite{yeshwanthliu2023scannetpp} test set. The Faro scanner point clouds act as a reference for the ground truth. All metrics are multiplied by $10^4$.}
	\centering
	\resizebox{\columnwidth}{!}{%
		\setlength{\tabcolsep}{3pt}
		\begin{tabular}{lccccccc|cccccc}
			\toprule
			& Input & \multicolumn{6}{c}{iPhone Reconstruction} & \multicolumn{6}{c}{3DMatch \cite{zeng20163dmatch} Reconstruction} \\
			\cmidrule(lr){3-8} \cmidrule(lr){9-14}
			Method                            & Features       & P2F      & F2P        & $\cdforw$ & $\cdbakw$  & CD        & P2M       & P2F       & F2P       & $\cdforw$ & $\cdbakw$ & CD        & P2M       \\
			\midrule
			Bilateral \cite{digne_bilateral}  & XYZ            & 6.29     & 140.59     & 6.66      & 145.44     & 73.44     & 76.05     & 108.70    & \st 18.32     & 108.89    & \st 19.67 & 64.28     & 63.51     \\
			DMR \cite{luo2020differentiable}  & XYZ            & 6.48     & 149.99     & 6.71      & 159.13     & 78.24     & 82.92     & 99.96     & 19.61     & 100.16    & 21.27     & 60.71     & 59.79     \\
			ScoreDenoise \cite{score_denoise} & XYZ            & 3.49     & \rd 128.59 & 3.72      & \rd 132.71 & 68.21     & 66.04     & 97.11     & 18.87     & 97.31     & 20.26     & 58.78     & 57.99     \\
			MAG \cite{zhao2023point}          & XYZ            & 5.43     & 147.54     & 5.66      & 152.07     & 78.87     & 76.49     & 99.05     & 24.82     & 99.26     & 26.69     & 62.97     & 61.93     \\
			PD-Flow \cite{mao2022pd}          & XYZ            & 3.80     & 147.49     & 4.02      & 151.90     & 77.96     & 75.64     & 85.29     & 21.00     & 85.49     & 22.56     & 54.02     & 53.14     \\
			\textbf{\name{} (Ours)}           & XYZ            & \rd 2.48 & \st 122.23 & \rd 2.71  & \st 126.22 & \nd 64.46 & \nd 62.35 & \rd 50.87 & 18.69 & \rd 51.07 & 20.05     & \rd 35.56 & \rd 34.78 \\
			\midrule
			\textbf{\name{} (Ours)}           & XYZ, RGB       & \nd 2.47 & \nd 122.27 & \nd 2.70  & \nd 126.26 & \rd 64.48 & \rd 62.37 & \nd 50.40 & \nd 18.39 & \nd 50.60 & \nd 19.73 & \nd 35.17 & \nd 34.39 \\
			\textbf{\name{} (Ours)}           & XYZ, RGB, DINO & \st 2.42 & \st 122.23 & \st 2.65  & \st 126.22 & \st 64.44 & \st 62.33 & \st 49.64 & \rd 18.57 & \st 49.84 & \rd 19.92 & \st 34.88 & \st 34.11 \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:evaluation_snpp}
\end{table}
